Readout technologies for directional WIMP Dark Matter detection

The measurement of the direction of WIMP-induced nuclear recoils is a compelling but technologically challenging strategy to provide an unambiguous signature of the detection of Galactic dark matter. Most directional detectors aim to reconstruct the dark-matter-induced nuclear recoil tracks, either in gas or solid targets. The main challenge with directional detection is the need for high spatial resolution over large volumes, which puts strong requirements on the readout technologies. In this paper we review the various detector readout technologies used by directional detectors. In particular, we summarize the challenges, advantages and drawbacks of each approach, and discuss future prospects for these technologies.

==> DDR_Authorlist.tex <==
% e.g.
% \author[\WellesleyCollege]{James~B.~R.~Battat,}
% \author[\UHawaii]{Sven~E.~Vahsen,}
% \author[\RoyalHolloway]{Jocelyn~Monroe,}
% \author[\KobeUniversity]{Kentaro~Miuchi,}

%\author[\AnotherInstitution]{Author~list~order~currently~arbitrary,%
%\note{Corresponding author.}}
%\author[\MyUniversity]{First~Author,}
%\author[\YetAnotherUniversity]{and Last~Author}

\author[\Wellesley]{J.~B.~R.~Battat,\note{Corresponding author.}}
\author[\UNIZAR]{I.~G.~Irastorza,}
\author[\INFNNapoli]{A.~Aleksandrov,}
\author[\METU]{M.~Ali Guler,}
\author[\Nagoya]{T.~Asada,} 
%\author[\MITLNS,\LBNL]{J.~Balewski,}
\author[\INFNLNF]{E.~Baracchini,}
\author[\LPSC,\IPNL]{J.~Billard,}
\author[\LPSC]{G.~Bosson,}
\author[\LPSC]{O.~Bourrion,}
\author[\LPSC]{J.~Bouvier,}
\author[\INFNNapoli,\Napoli]{A.~Buonaura,}
\author[\MITLNS,\CALTECH]{K.~Burdge,}
\author[\UNIZAR]{S.~Cebri\'{a}n,}
\author[\CEA]{P.~Colas,}
\author[\INFNLNGS]{L.~Consiglio,} 
%\author[\MITLNS]{R.~Corliss,}
\author[\UNIZAR]{T.~Dafni,}
\author[\INFNLNGS]{N.~D'Ambrosio,}
\author[\MITLNS,\UCHICAGONOW]{C.~Deaconu,}
\author[\INFNNapoli,\Napoli]{G.~De Lellis,}
\author[\LPSC]{T.~Descombes,}
\author[\INFNNapoli]{A.~Di Crescenzo,}
%\author[\MITLNS]{H.~Diehl,}
\author[\INFNLNGS]{N.~Di Marco,}
\author[\RHUL]{G.~Druitt,}
\author[\RHUL]{R.~Eggleston,}
\author[\CEA]{E.~Ferrer-Ribas,}
%\author[\MITPHYS,\MITKAVLI,\MITLNS]{P.~Fisher,}
%\author[\Nagoya]{S.~Furuya,}
\author[\sagaUniversity]{T.~Fusayasu,}
\author[\UNIZAR]{J.~Gal\'{a}n,}
\author[\INFNNapoli,\Napoli]{G.~Galati,}
\author[\UNIZAR]{J.~A.~Garc\'{i}a,}
\author[\UNIZAR]{J.~G.~Garza,}
\author[\INFNGranSasso]{V.~Gentile,}
\author[\LBNL]{M.~Garcia-Sciveres,}
\author[\CEA]{Y.~Giomataris,}
\author[\RHUL,\MITLNS]{N.~Guerrero,}
\author[\LPSC]{O.~Guillaudin,}
\author[\CSU]{J.~Harton,}
\author[\KobeUniversity]{T.~Hashimoto,}
\author[\HAWAII]{M.~T.~Hedges,}
\author[\UNIZAR]{F.~Iguaz,}
\author[\KobeUniversity]{T.~Ikeda,}
\author[\UFL]{I.~Jaegle,} 
\author[\LBNL]{J.~A.~Kadyk,}
\author[\Nagoya]{T.~Katsuragawa,}
%\author[\Nagoya]{M.~Kimura,}
\author[\kyotouniversity]{S.~Komura,}
\author[\kyotouniversity]{H.~Kubo,}
\author[\Chiba]{K.~Kuge,}
\author[\LPSC]{J.~Lamblin,}
\author[\INFNNapoli,\Napoli]{A.~Lauria,}
\author[\UNM]{E.~R.~Lee,}
\author[\HAWAII]{P.~Lewis,}
\author[\RHUL,\MITLNS]{M.~Leyton,}
\author[\UNM]{D.~Loomba,}
\author[\MITLNS,\UCOLORADO]{J.~P.~Lopez,}
\author[\UNIZAR]{G.~Luz\'{o}n,}
%\author[\Nagoya]{S.~Machii,}
%\author[\kyotouniversity]{Y.~Matsuoka,}
\author[\LPSC]{F.~Mayet,}
\author[\UNIZAR]{H.~Mirallas,}
\author[\KobeUniversity]{K.~Miuchi,} 
\author[\kyotouniversity]{T.~Mizumoto,}
\author[\kyotouniversity]{Y.~Mizumura,}
\author[\INFNRoma]{P.~Monacelli,} 
\author[\RHUL,\kekTsukuba]{J.~Monroe,}
\author[\INFNNapoli,\Napoli]{M.~C.~Montesi,}
\author[\Nagoya]{T.~Naka,} 
\author[\kyotouniversity]{K.~Nakamura,}
\author[\kyotouniversity]{H.~Nishimura,}
\author[\KobeUniversity]{A.~Ochi,} 
\author[\CEA]{T.~Papevangelou,}
\author[\NSTC]{J.D.~Parker,}
\author[\UNM]{N.~S.~Phan,}
\author[\INFNLNGS]{F.~Pupilli,}
\author[\LPSC]{J.~P.~Richer,}
\author[\PARIS]{Q.~Riffard,}
\author[\Roma,\INFNRoma]{G.~Rosa,}
\author[\LPSC]{D.~Santos,}
\author[\kyotouniversity]{T.~Sawano,}
\author[\kamiokaObservatory]{H.~Sekiya,}
\author[\HAWAII]{I.~S.~Seong,}
\author[\OXY]{D.~P.~Snowden-Ifft,}
\author[\Sheffield]{N.~J.~C.~Spooner,}
\author[\sagaUniversity]{A.~Sugiyama,}
\author[\KobeUniversity]{R.~Taishaku,} 
\author[\kyotouniversity]{A.~Takada,}
\author[\kamiokaObservatory]{A.~Takeda,}
\author[\kekTsukuba]{M.~Tanaka,}
\author[\kyotouniversity]{T.~Tanimori,}
\author[\HAWAII]{T.~N.~Thorpe,}
\author[\INFNNapoli]{V.~Tioukov,}
\author[\MITLNS,\SILVERSIDE]{H.~Tomita,}
\author[\Nagoya]{A.~Umemoto,}
\author[\HAWAII]{S.~E.~Vahsen,}
\author[\KobeUniversity]{Y.~Yamaguchi,}
\author[\Nagoya]{M.~Yoshimoto,}
\author[\MITLNS]{and E.~Zayas}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AFFILIATIONS 
\affiliation[\Wellesley]{Department of Physics, Wellesley College, 106 Central Street, Wellesley, MA 02481, USA}
\affiliation[\UNIZAR]{Grupo de F\'{i}sica Nuclear y Astropart\'{i}culas, Departamento de F\'{i}sica Te\'{o}rica, Universidad de Zaragoza, 50009 Zaragoza, Spain}
%\affiliation[\INFNNapoli]{INFN Sezione di Napoli, I-80125 Napoli, Italy} 
\affiliation[\INFNNapoli]{Istituto Nazionale di Fisica Nucleare, Sezione di Napoli, Naples, Italy}
\affiliation[\METU]{METU Middle East Technical University, TR-06531 Ankara, Turkey} 
\affiliation[\Nagoya]{Nagoya University, J-464-8602 Nagoya, Japan}
%\affiliation[\INFNLNF]{INFN - Laboratori Nazionali di Frascati dell'INFN, I-00044 Frascati (Roma), Italy} 
\affiliation[\INFNLNF]{Istituto Nazionale di Fisica Nucleare, Laboratori Nazionali di Frascati, Frascati, Italy}
\affiliation[\LPSC]{Laboratoire de Physique Subatomique et de Cosmologie, Universit\'e Grenoble Alpes, CNRS/IN2P3, 53, avenue des Martyrs, Grenoble, France}
\affiliation[\IPNL]{IPNL, Universit\'{e} de Lyon, Universit\'{e} Lyon 1, CNRS/IN2P3, 4 rue E. Fermi 69622 Villeurbanne cedex, France}
\affiliation[\Napoli]{Dipartimento di Fisica, Universit\`{a} Federico II, Napoli, I-80125 Napoli, Italy} 
\affiliation[\MITLNS]{Laboratory for Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\affiliation[\CALTECH]{Caltech Division of Physics, Mathematics, and Astronomy, Pasadena, CA, USA}
\affiliation[\CEA]{IRFU, CEA, Universit\'{e} Paris-Saclay, Gif-sur-Yvette, France}
\affiliation[\CSU]{Department of Physics, Colorado State University, Fort Collins, CO 80523-1875, USA}
%\affiliation[\INFNLNGS]{Laboratori Nazionali del Gran Sasso, I-67010 Assergi (L'Aquila), Italy}
\affiliation[\INFNLNGS]{Istituto Nazionale di Fisica Nucleare, Laboratori Nazionali del Gran Sasso, Assergi, Italy}
%\affiliation[\MITPHYS]{Physics Department, Massachusetts Institute of Technology, Cambridge, MA 02138, USA}
%\affiliation[\MITKAVLI]{MIT Kavli Institute for Astrophysics and Space Research, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\affiliation[\UCHICAGONOW]{University of Chicago, Kavli Institute for Cosmological Physics, Chicago, IL, USA}
\affiliation[\RHUL]{Department of Physics, Royal Holloway, University of London, Egham Hill, Surrey, TW20 0EX, UK}
\affiliation[\sagaUniversity]{Department of Physics, Faculty of Science and Engineering, Saga University, Saga, 840-8502, Japan }
\affiliation[\INFNGranSasso]{Gran Sasso Science Institute (INFN), L'Aquila, Italy}
\affiliation[\LBNL]{Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720, USA}
\affiliation[\KobeUniversity]{Department of Physics, Kobe University, Rokodai, Nada-ku Kobe-shi, Hyogo, 657-8501, Japan}
\affiliation[\HAWAII]{University of Hawaii, 2505 Correa Road, Honolulu, HI 96822, USA}
\affiliation[\UFL]{University of Florida, Department of Physics, P.O. Box 118440, Gainesville, FL 32611, USA}
\affiliation[\kyotouniversity]{Department of Physics, Kyoto University, Oiwakecho, Sakyo-ku Kyoto-shi, Kyoto, 606-8502, Japan}
\affiliation[\Chiba]{Chiba University, J-263-8522, Chiba, Japan} 
\affiliation[\UNM]{Physics \& Astronomy Department, University of New Mexico, 1919 Lomas Blvd NE, Albuquerque, NM 87131, USA}
\affiliation[\UCOLORADO]{University of Colorado, Department of Physics, Boulder, CO, USA}
%\affiliation[\INFNRoma]{INFN Sezione di Roma, I-00185 Roma, Italy}
\affiliation[\INFNRoma]{Istituto Nazionale di Fisica Nucleare, Sezione di Roma, Rome, Italy}
\affiliation[\kekTsukuba]{Institute of Particle and Nuclear Studies, KEK, 1-1 Oho,Tsukuba, Ibaragi, 305-0801, Japan}
\affiliation[\NSTC]{Neutron Science and Technology Center, Comprehensive Research Organization for Science and Society, Tokai-mura, Ibaraki, 319-1106, Japan}
\affiliation[\PARIS]{APC, Universit\'e Paris Diderot, CNRS/IN2P3, CEA/Irfu, Obs de Paris, Sorbonne Paris Cit\'e, 75205 Paris, France}
\affiliation[\Roma]{Dipertmento di Fisica dell'Universit a di Roma Sapienza, I-00185 Roma, Italy}
\affiliation[\kamiokaObservatory]{Kamioka Observatory, ICRR, The University of Tokyo, Gifu, 506-1205 Japan}
\affiliation[\OXY]{Department of Physics, Occidental College, Los Angeles, CA 90041, USA}
\affiliation[\Sheffield]{Department of Physics and Astronomy, University of Sheffield, S3 7RH, UK}
\affiliation[\SILVERSIDE]{Silverside Detectors Inc., Cambridge, MA, USA}

%\affiliation[\MyUniversity]{Department, University A,\\
%Street Number, City, Country}
%\affiliation[\AnotherInstitution]{Institution B,\\
%Street Number, City, Country}
%\affiliation[\YetAnotherUniversity]{Department, University C,\\
%Street Number, City, Country}

\emailAdd{jbattat@wellesley.edu}

